Swift4D:Adaptive divide-and-conquer Gaussian Splatting for compact and efficient reconstruction of dynamic scene

Novel view synthesis has long been a practical but challenging task, although the introduction of numerous methods to solve this problem, even combining advanced representations like 3D Gaussian Splatting, they still struggle to recover high-quality results and often consume too much storage memory and training time. In this paper we propose Swift4D, a divide-and-conquer 3D Gaussian Splatting method that can handle static and dynamic primitives separately, achieving a good trade-off between rendering quality and efficiency, motivated by the fact that most of the scene is the static primitive and does not require additional dynamic properties. Concretely, we focus on modeling dynamic transformations only for the dynamic primitives which benefits both efficiency and quality. We first employ a learnable decomposition strategy to separate the primitives, which relies on an additional parameter to classify primitives as static or dynamic. For the dynamic primitives, we employ a compact multi-resolution 4D Hash mapper to transform these primitives from canonical space into deformation space at each timestamp, and then mix the static and dynamic primitives to produce the final output. This divide-and-conquer method facilitates efficient training and reduces storage redundancy. Our method not only achieves state-of-the-art rendering quality while being 20X faster in training than previous SOTA methods with a minimum storage requirement of only 30MB on real-world datasets. Code is available at https://github.com/WuJH2001/swift4d.

==> iclr_rebuttal.tex <==


% 9PWz  5  4
% 这篇论文总体写得很好并且易于理解。作者提供了方法和实验的详细描述。
% 根据定量评估，该方法在图像质量和优化时间方面优于竞争方法。
% 这个想法相对简单，静态和动态分解，但在速度方面似乎是有效的。

% A key component of this work is the dynamic and static decomposition. The method introduces a dynamic level parameter that is optimized for each gaussian. As explained in section 3.2, a 2D dynamic-static pixel Mask is computed from the training video by leveraging the temporal standard deviation of each pixel. However, since the video can have camera motion as well as dynamic elements that yield varying the pixel intensity it is unclear to me how the standard deviation can serve as good criterion to differentiate dynamic scene elements from static ones. Does this criterion work well on videos with strong camera motion?

% The authors propose a temporal pruning strategy, it would be good to discuss at some point existing pruning strategies, e.g. LightGaussians (Fan et al. NeurIPS 2024), and the relation ship the proposed pruning method.
% In the supplementary material videos, there seem to be artifacts of vanishing dynamic elements. In 2_baskball2.mp4 some players vanishing from frame to frame and it appears to have temporal inconsistencies, that questions the effectiveness of the method. Is this a common issue?

% How can the model differentiate between specular reflections and dynamic elements?

% Q1: 这项工作的一个关键组成部分是动态和静态分解。该方法引入了针对每个高斯优化的动态水平参数。如 3.2 节中所述，2D 动态-静态像素掩模是通过利用每个像素的时间标准差从训练视频计算得出的。然而，由于视频可能具有摄像机运动以及产生不同像素强度的动态元素，因此我不清楚标准差如何作为区分动态场景元素和静态场景元素的良好标准。此标准对于摄像机运动强烈的视频是否有效？

% Q2: 作者提出了一种时间剪枝策略，最好在某个时候讨论现有的剪枝策略，例如LightGaussians (Fan et al. NeurIPS 2024)，以及所提出的剪枝方法的关系。

% Q3: 在补充材料视频中，似乎存在动态元素消失的伪影。在 2_baskball2.mp4 中，一些玩家从帧到帧消失，并且似乎存在时间不一致，这质疑该方法的有效性。这是一个常见问题吗？

% Q4: 模型如何区分镜面反射和动态元素？



% 感谢你的细心审稿，我们将针对你的concern的问题进行逐一回答
%   Q1: 实际上和之前的一些方法一样【】，我们的方法主要关注多视图场景，在这些数据集中不存在摄像机运动的问题，因此我们并没有考虑运动相机的情况。我们方法设计的底层逻辑在于：在多视图场景中相机固定，如果像素光线与动态物体存在交集，那么这个像素会出现剧烈的改变，其标准差也会偏大。反过来，我们根据这个思路，如果像素标准差较大，那么和其相交的高斯点理应更倾向于动态，反之倾向于静态。标准差就是根据这个思路区分场景中动静态元素。
%   Q2: 我们将在对应的章节讨论不同点，并且在 PDF 文件修改
%   Q3: 实际上我们是第一个在如此大规模的动态数据集上进行实验，消失、闪烁问题的主要原因是这个数据集更为复杂，运动幅度更大，这是目前动态方法普遍存在的问题。并且我们也提供了其他方法的训练结果，包括流式的3DGStream和非流式的 4DGS。我们的方法虽然也存在一定的闪烁问题，但是相比于他们的方法能够更忠实的表示运动。关于帧间不一致问题是因为一个时域模型难以对这么大的场景进行长序列的动态建模（这个问题是普遍存在的），因此我们每20帧重新构建一个时域结构，从而导致每20帧会出现一次闪烁问题。

%   Q4: 虽然目前的动态方法中没有人考虑镜面反射这个问题。但是我们很乐意去探讨这个问题，根据我们的设计思路，如果在某个视角下，观测到镜子反射了运动的物体，那么在镜子区域将会存在动态的高斯点对镜面反射的动态物体进行建模。我们并没有针对镜面反射进行特殊处理，根据我们的设计思路，我们采用像素方差作为监督，只要像素点存在改变，那么对应的高斯点就会倾向于变为动态。

Thank you for your review. We will make improvements based on your feedback. Next, we will address your concerns point by point. If there are any areas where our explanations are unclear, please feel free to point them out.

**W1: However, since the video can have camera motion as well as dynamic elements that yield varying the pixel intensity it is unclear to me how the standard deviation can serve as good criterion to differentiate dynamic scene elements from static ones.**

Dynamic scene reconstruction methods are divided into two approaches: monocular video input (with camera motion, e.g., SCGS [10], DeformableGS [9]) and multi-view video input (without camera motion, e.g., 3DGStream [1], SpaceTimeGS [3]), each posing unique challenges.

The "videos with camera motion" you mentioned may fall into the category of monocular videos. However, similar to previous works [1, 3], our method focuses on multi-view scene reconstruction, where the cameras are fixed, and no camera motion occurs. Therefore, the concern you raised about "camera motion causing...static elements" has not been considered in our approach, as it primarily targets multi-view datasets where camera motion is absent.

Upon further reflection, as Reviewer-9PWz pointed out, if camera motion exists (in monocular videos), the standard deviation is indeed not a reliable criterion for distinguishing dynamic scene elements from static ones. However, results from mainstream multi-view datasets, such as N3DV [11], MeetRoom [12], and our VRU [13] dataset, demonstrate that the standard deviation serves as an effective supervision signal for multi-view input.


**W2: Does this criterion work well on videos with strong camera motion?**

Aligned with previous works (3DGStream [1], SpaceTime [3]), a limitation of our method, as well as theirs, is its focus on multi-view dynamic scene reconstruction ( without camera motion), making it unsuitable for reconstructing dynamic scenes from monocular videos ( with strong camera motion ). Consequently, our method is not applicable to monocular dynamic datasets with camera motion. 

**W3: Discuss the differences between our approach and existing pruning strategies.**

Thank you for your suggestions. We will elaborate on the differences in the relevant section and implement the changes in the PDF file as outlined below. 

**LightGS[8] prunes Gaussian points in the spatial domain based on attributes such as opacity and volume. In contrast, our method focuses on pruning Gaussian points based on their importance across all training views in the entire temporal domain.**


**W4:  there seem to be artifacts of vanishing dynamic elements. In 2_baskball2.mp4 some players vanishing from frame to frame and it appears to have temporal inconsistencies.**

**Temporal inconsistencies**: The basketball video we provided is composed of several 20-frame video clips stitched together, which may result in frame-to-frame inconsistencies. These inconsistencies are not caused by our method. 

**Artifacts of disappearing dynamic elements**: We are the first to experiment with such a large-scale dynamic dataset. The main cause of issues like disappearance and flickering is the dataset's increased complexity and larger motion amplitudes, which is common in current dynamic methods. **We have provided VRU training results from other methods in the Supplementary Material, including the online 3DGStream[1] and offline 4DGS[2].** 

**W5: How can the model differentiate between specular reflections and dynamic elements?**

Specular reflections are a challenging problem [4,5,6]. While current dynamic methods don't address them, we are open to exploring this issue. Our method currently cannot distinguish specular reflections from dynamic elements. If a moving object is reflected in a mirror, it treats the reflection as dynamic, marking the Gaussians in the mirror region to model the changes.

Finally, we sincerely thank you for your questions. Your insights have indeed helped us further refine our paper.

**Reference**

[1] 3DGStream: On-the-fly Training of 3D Gaussians for Efficient Streaming of Photo-Realistic Free-Viewpoint Videos. CVPR 2024

[2] 4D Gaussian Splatting for Real-Time Dynamic Scene Rendering. CVPR 2024.

[3] Spacetime Gaussian Feature Splatting for Real-Time Dynamic View Synthesis. CVPR 2024.

[4] SpecNeRF: Gaussian Directional Encoding for Specular Reflections. CVPR 2024.

[5] Spec-Gaussian: Anisotropic View-Dependent Appearance for 3D Gaussian Splatting. NIPS 2024.

[6] MirrorGaussian: Reflecting 3D Gaussians for Reconstructing Mirror Reflections. ECCV 2024.

[7] Segment Anything. ICCV 2023.

[8] LightGaussian: Unbounded 3D Gaussian Compression with 15x Reduction and 200+ FPS. NIPS 2024.

[9] Deformable 3D Gaussians for High-Fidelity Monocular Dynamic Scene Reconstruction. CVPR 2024.

[10] SC-GS: Sparse-controlled Gaussian splatting for editable dynamic scenes. CVPR 2024.

[11] Neural 3d video synthesis from multi-view video. CVPR 2022.

[12] Streaming radiance fields for 3d video synthesis. NIPS 2022.

[13] VRU. https://anonymous.4open.science/r/vru-sequence/. 2024.

\newpage



%  6 4
% 本文的动机和技术设计简单合理。在处理真实的动态场景时，静态和动态内容解耦是一种直观的方法。尽管该方法存在疑问，但它可能有助于研究人员更好地理解问题并利用 3DGS 的显式结构。
% 不同数据集上的实验结果显示了各个方面的改进，例如训练时间和 PSNR，尽管 FPS 较低，而且这不是一种动态方法。
% 这篇论文的写作和插图对我来说非常清楚。

% One critical weakness is the implementation of decoupling static and dynamic parts. Specifically, they use 2D supervision to build the dynamic factor. However, the way they build 2D masks is just to calculate the temporal variance of each pixel, which should lead to problems when dynamic movements happen in textureless regions. These regions can easily be recognized as static parts. Such a phenomenon could be observed in the sear_steak_static result of the supplementary, where part of the cloth is classified as static. In addition, calculating the variance throughout the entire time could cause problems in long-sequence video.

% It seems that this work can't deal with single-view videos like DNeRF. This could be a general limitation as it's hard to deploy and compare with other methods that can deal with such cases (e.g., SCGS). In addition, it needs to be trained offline, making the comparison with 3DGSStream kind of unfair.

% To me, the result in Fig.7 does actually demonstrate the sensitivity of the dynamic threshold, where it affects the PSNR a lot. I am worried about the generalizability of the method since it's tested on scenes with similar dynamic-static compositions.

% As described in weakness, my questions mainly focus on the generalizability to texture-less regions, highly dynamic videos (with different static-dynamic compositions), and long-term videos.

% Q1：一个关键的弱点是静态和动态部分解耦的实现。具体来说，他们使用 2D 监督来构建动态因子。然而，他们构建 2D 掩模的方式只是计算每个像素的时间方差，当动态运动发生在无纹理区域时，这会导致问题。这些区域很容易被识别为静态部分。这种现象可以在补充的 sear_steak_static 结果中观察到，其中部分布料被归类为静电。此外，计算整个时间的方差可能会导致长序列视频出现问题。

% Q2: 看来这项工作无法处理像DNeRF这样的单视图视频。这可能是一个普遍的限制，因为它很难部署并与可以处理此类情况的其他方法（例如 SCGS）进行比较。此外，它需要离线训练，这使得与 3DGSStream 的比较有点不公平。

% Q3: 对我来说，图 7 中的结果确实证明了动态阈值的敏感性，它对 PSNR 影响很大。我担心该方法的普遍性，因为它是在具有类似动态-静态构图的场景上进行测试的。

% Q4: 正如弱点中所述，我的问题主要集中在无纹理区域、高动态视频（具有不同的静态动态组合）和长期视频的通用性上。


% Q1: 实际上我们已经在 Discussion 讨论了这个问题，我们可以将弱纹理动态元素分为两类：一种是具有large-scale 运动的弱纹理动态元素，一种是 fine-scale 运动的弱纹理元素。
% 对于第一种，可以看到我们补充的视频 1_basketball，运动员身上的弱纹理衣服其实被归类为动态元素，和运动员一起进行形变。
% 对于第二种，使用2D 掩膜作为监督的确会将一部分运动有限的弱纹理动态元素识别为静态，比如衣料，桌子的中心区域，但是对于其边缘区域仍会识别为动态，可以在补充的 sear_steak_dynamic 可以看到。而这些弱纹理物体的中心区域分类为静态其实不会有任何的影响. 即使我们采用 SAM 作为监督，将这部分识别为动态，对这些颜色一样的高斯点进行形变或者不形变也不会对渲染结果有任何改变，因此将其识别为静态是合理的。
% 实际上，我们只是为了不引入更多的外部先验，所以才采用时间方差作为监督，如果为了适应长序列视频，我们可以考虑直接使用 SAM 提供良好的先验，分割出动态物体。 

% Q2: 是的，我们的方法和一些论文一样【】聚焦于多视图动态场景重建。我们将把 3DGStream单独进行标记为在线方法进行区分。
% Q3：实际上，我们在所有的实验上都设置阈值为 7.0，并没有单独调节阈值，我们的方法都能够达到一个良好的性能优势。

% Q4: 对于高动态视频和长序列视频的通用性




Thank you very much for your recognition and valuable feedback. Here, we will address your concerns point by point. If there are any areas where our explanations are unclear, please feel free to point them out.

**W1: Using the 2D mask calculated from the temporal variance of pixels as supervision may lead to issues when dynamic motion occurs in textureless areas. These regions can easily be recognized as static parts.**


We can classify weak-texture dynamic elements into two categories: one is weak-texture dynamic elements with large-scale motion, and the other is weak-texture elements with fine-scale motion.

For the first category, as seen in our supplementary video 1 basketball, the weak-texture clothing worn by the athlete is classified as a dynamic element and deforms along with the athlete's movement. Therefore, our method performs well in such situations.

For the second category, using 2D masks as supervision can indeed lead to some weak-texture dynamic elements with limited motion being classified as static, such as the central area of fabric. 
However, this issue only occurs in the central area of textureless item (fabric), while the dynamic classification still holds for the edges of these elements, as seen in the supplementary video sear_steak_dynamic. In fact, whether the Gaussian points in the central region of weak-texture objects with fine-scale motion are classified as dynamic or static, the rendering results remain the same. Because they have the same color, their internal motion does not affect the rendering results, regardless of how they move.

Therefore, using the 2D mask calculated from the temporal variance of pixels as supervision is reasonable.

Additionally, the choice of supervision signal is flexible; it can be the 2D mask calculated from the temporal variance of pixels, SAM [1], or other methods. We simply provide a basic approach using variance as supervision.



**W2: Calculating the variance throughout the entire time could cause problems in long-sequence video.**

We are not clear on the specific problems you are referring to. Please allow us to respond based on our interpretation of the issue.

We classify long-sequence videos into two categories: those capturing small-scale motions and those capturing large-scale motions.

For the first category(small-scale motions), the static background remains unchanged and occupies most of the scene, while dynamic objects are confined to small moving regions within the scene. In such cases, there is essentially no difference between long and short video sequences; both have only a small portion of dynamic pixels exhibiting high temporal variance, while the majority of pixels display low variance. Under these circumstances, calculating variance as a supervision signal works equally well for both long and short sequences, without any issues.


For the second category(large-scale motions), while the static background still occupies a significant portion, the dynamic objects exhibit extensive movement, which can cause all pixels to display high variance and be marked as dynamic pixels. In such cases, as reviewer have pointed out, our dynamic-static separation method may fail due to inaccurate supervision signals. To address this issue, using SAM [1] as a supervision signal to directly identify and extract dynamic objects could be a promising solution.


Currently, results from mainstream multi-view datasets like N3DV [2], MeetRoom [3], and our VRU [9] dataset suggest that calculating the variance across the entire timeline poses no issues. 


Additionally, directly performing dynamic reconstruction on long-sequence videos is uncommon, as these videos require storing a large amount of dynamic information, which is difficult to represent within a single temporal structure. This often results in severe blurring and flickering issues. **A common and practical solution is to divide them into shorter sequences and perform dynamic reconstruction on each sequence individually, where calculating the variance poses no issues.**


**W3:  It seems that this work can't deal with single-view videos like DNeRF. This could be a general limitation as it's hard to deploy and compare with other methods that can deal with such cases (e.g., SCGS).**


Yes, similar to 3DGStream[4] and SpaceTimeGS[5], our method focuses on multi-view dynamic scene reconstruction and can not  handle single-view videos like D-NeRF. In contrast, SCGS[8] and D-NeRF[6] focus more on monocular datasets and struggle to handle multi-view datasets well [2,3]. All of these methods tackle different tasks, making a direct comparison between them challenging. Both monocular and multi-view dynamic scene reconstruction come with their own challenges.


**W4: In addition, it needs to be trained offline, making the comparison with 3DGSStream kind of unfair.**

Yes, our method is trained offline, and we will specifically label 3DGStream as an online training method.


**W5: To me, the result in Fig.7 does actually demonstrate the sensitivity of the dynamic threshold, where it affects the PSNR a lot.**

Considering reviewer's concern, the PSNR could fluctuate slightly with small adjustments in the threshold due to the smaller size of the N3DV datasets[2]. Therefore, we conducted ablation experiments on the VRU basketball court dataset[9], which has a larger dynamic range and coverage. The experimental results are as follows:

| Dynamic Threshold | PSNR   | Dynamic-Static Compositions |
|--------------------|--------|----------------------------|
| 3.0               | 28.76  | 0.230                      |
| 4.0               | 28.89  | 0.215                      |
| 5.0               | 28.82  | 0.204                      |
| 6.0               | 28.81  | 0.187                      |
| 7.0               | 29.10  | 0.173                      |
| 8.0               | 28.62  | 0.163                      |
| 9.0               | 28.57  | 0.138                      |


**W6: Worried about the generalizability of the method since it's tested on scenes with similar dynamic-static compositions.**


In fact, our dynamic-static separation approach is specifically designed for scenarios where the static portion is large (over 70%) and the dynamic portion is small (10%-30%). This dynamic-static composition closely mirrors real-world scenes, and our method has proven to be highly effective.

If a scene, as pointed out by the reviewer, has a different dynamic-static composition (with the dynamic proportion being large, 70% or even higher), then applying a dynamic-static separation strategy may not be necessary. Directly modeling the entire scene might be more reasonable in such cases. In such cases, applying our dynamic-static separation approach may not yield significant benefits, as the performance gains from reducing the computational load on the static part are limited when the dynamic portion is large. 

Considering the reviewer’s concerns, we tested our method on the VRU dataset, where the dynamic-static compositions exhibit varying distributions (ranging from 0.138 to 0.230) based on adjustments to the dynamic threshold.


| Dynamic Threshold | PSNR   | Dynamic-Static Compositions |
|--------------------|--------|----------------------------|
| 3.0               | 28.76  | 0.230                      |
| 4.0               | 28.89  | 0.215                      |
| 5.0               | 28.82  | 0.204                      |
| 6.0               | 28.81  | 0.187                      |
| 7.0               | 29.10  | 0.173                      |
| 8.0               | 28.62  | 0.163                      |
| 9.0               | 28.57  | 0.138                      |


**Others:**

**Inadditional, we have provided training results from other methods in the Supplementary Material, including the online 3DGStream[1] and offline 4DGS[2].** 

Finally, we sincerely thank you for your questions. Your insights have indeed helped us further refine our paper.




**Reference**

[1] Segment Anything. ICCV 2023.

[2] Neural 3d video synthesis from multi-view video. CVPR 2022.

[3] Streaming radiance fields for 3d video synthesis. NIPS 2022.

[4] 3dgstream: On-the-fly training of 3d gaussians for efficient streaming of photo-realistic free-viewpoint videos

[5] Spacetime Gaussian Feature Splatting for Real-Time Dynamic View Synthesis. CVPR 2024.

[6] D-NeRF: Neural Radiance Fields for Dynamic Scenes. CVPR 2021.

[7] Deformable 3D Gaussians for High-Fidelity Monocular Dynamic Scene Reconstruction. CVPR 2024.

[8] SC-GS: Sparse-controlled Gaussian splatting for editable dynamic scenes. CVPR 2024.

[9] VRU. https://anonymous.4open.science/r/vru-sequence/. 2024.




%  VRU  114899 / 400000    28.76  3.0
%       107319 / 708819    28.89  4.0
%        102452 / 703887     28.82  5.0
%        93644 / 695941    28.81  6.0 
%        86622 / 691356    29.10   7.0
%        81652 /703549     28.62   8.0
%         69176/ 686444    28.57   9.0








\newpage



% 6  5

% 分解静态和动态元素是有益的，可以有效减轻模型的学习负担并提高推理速度，如表3所示。值得注意的是，这种分离也存在于并行工作 GauFRe（Liang等人）和已发表的工作SC-GS中（黄等人）。这个概念是对 GauFRe 的重大贡献，也是 SC-GS 中的详细实现。在讨论这个想法时引用这些方法是合适的。

% 3.4节中的剪枝策略是创新的。 Gaussian Splatting 和 NeRF 基于多视图立体 (MVS) 原理，当多视图图像达到光度一致性时会收敛。一个孤立的高斯点，仅被少数视图识别，往往会成为浮动伪影，导致过度拟合。这一富有洞察力的观点很有价值，并且能够激励社区。


% The experimental results and citations are insufficient. The FPS of Swift4DLite (Ours) is missing in Table 1, with no explanation provided. Additionally, the rendering speed is relatively slow, similar to 4DGS (Yang et al.) and SpaceTimeGS, with comparable rendering quality. The training time for SpaceTimeGS reported in Table 1 is too long; it should be under an hour. The FPS of SpaceTimeGS is also lower than I expected (130+). Moreover, several closely related works are not compared or cited:

% Huang, Yi-Hua, et al. "SC-GS: Sparse-controlled Gaussian splatting for editable dynamic scenes." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2024.
% Yang, Ziyi, et al. "Deformable 3D Gaussians for high-fidelity monocular dynamic scene reconstruction." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2024.
% Lin, Youtian, et al. "Gaussian-flow: 4D reconstruction with dynamic 3D Gaussian particles." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2024.

% I recommend at least including comparisons with (1) and (3), as these methods model Gaussian dynamics using spatially and frequency-compact bases, respectively. Additionally, SC-GS achieves high FPS in rendering images by inferring the motion of sparse control points, according to their Supp.


% 实验结果和引用不够充分。表 1 中缺少 Swift4DLite（我们的）的 FPS，且未提供任何解释。此外，渲染速度相对较慢，类似于4DGS（Yang等人）和SpaceTimeGS，但渲染质量相当。表1中报告的SpaceTimeGS的训练时间太长；应该不到一个小时。 SpaceTimeGS 的 FPS 也低于我的预期（130+）。而且，几个密切相关的作品没有进行比较或引用：
% 黄宜华，等。 “SC-GS：用于可编辑动态场景的稀疏控制高斯泼溅。” IEEE/CVF 计算机视觉和模式识别会议论文集。 2024 年。
% 杨子仪，等。 “用于高保真单目动态场景重建的可变形 3D 高斯。” IEEE/CVF 计算机视觉和模式识别会议论文集。 2024 年。
% 林友田，等。 “高斯流：使用动态 3D 高斯粒子进行 4D 重建。” IEEE/CVF 计算机视觉和模式识别会议论文集。 2024 年。
% 我建议至少包括与（1）和（3）的比较，因为这些方法分别使用空间和频率紧凑基来模拟高斯动力学。此外，根据他们的补充材料，SC-GS 通过推断稀疏控制点的运动来实现渲染图像的高 FPS。




% 非常感谢您的认可，我们将针对你提出的意见进行修改。
% Q1 缺少FPS： 非常抱歉让你产生了困扰，缺少的 Swift4DLite 的FPS是因为和 缺少 Swift4D 接近，所以省略，我们将修改论文。

% Q2: 表1中报告的SpaceTimeGS的训练时间太长；应该不到一个小时。 SpaceTimeGS 的 FPS 也低于我的预期（130+）。
% 实际上他们论文报告的训练时间是在  RTX A6000 上 50 帧图像的训练时间（ AS shown In their paper Sec.5 Implementation Details），但是我们在 RTX 3090 训练发现他们训练时间大概在 1.5-2h 训练50帧，而我们主流的是测试300帧的训练时间，他们总共需要 10 h 左右，远远超过我们的25分钟。对于FPS 我们忠实的报告我们在 3090 测试结果，可能存在一定的显卡性能差异。

% Q3: 渲染速度相对较慢：实际上我们的 FPS 是125，相比于 4DGS（Yang等人）和SpaceTimeGS 略高

% Q4: 几个密切相关的作品没有进行比较或引用。
% 【1】【2】的工作主要聚焦于单目视频，而我们的方法和3DGStream一样聚焦于多目视频，因此我们不太容易与他们进行比较，我们会在论文说明这个差别。对于【3】，我们将在论文报告他们的结果，并且我们补充了他们在主流多目数据集NV3D上的的训练结果.



Thank you very much for your recognition. We will address your concerns point by point and revise the paper based on your suggestions.

**W1:  The FPS of Swift4DLite (Ours) is missing in Table 1, with no explanation provided.**

The missing FPS for Swift4DLite is omitted because it is close to that of Swift4D. We will modify the paper accordingly.

**W2: The rendering speed is relatively slow, similar to 4DGS (Yang et al.) and SpaceTimeGS, with comparable rendering quality.**

Yes, our rendering speed is indeed similar to theirs, but our method actually achieves 125 FPS on dynamic scene datasets (Resolution: 1352x1014), which, to the best of our knowledge, is currently the highest performance.

**W3: The training time of SpaceTimeGS reported in Table 1 is too long; it should be under an hour. The FPS of SpaceTimeGS is also lower than my expectations (130+).**

Actually, the training time reported in their paper is based on training 50 frames on an **RTX A6000** (as shown in Section 5: Implementation Details of their paper). However, during our training on the **NVIDIA RTX 3090**, we find that their reported training time for 50 frames is around 1.5-2 hours. Therefore, their total training time for 300 frames would be approximately 10 hours. As for FPS, we faithfully report the results from our NVIDIA RTX 3090 tests. The difference between our results and those reported in their paper may be due to the difference in GPU models.


**W4: Several closely related works have not been compared or cited.**

SC-GS [1] is indeed a work closely related to ours and achieves very high FPS and rendering quality. However, they [1,2] seem to focus more on monocular dynamic scene reconstruction, while we focus on multi-view dynamic scene reconstruction. Therefore, comparing our work with these two studies presents certain challenges. We will also explain this point in the paper.

As for [3], we will report their results in the paper. Their results on the mainstream multi-view dataset N3DV [6] are as follows.

method | PSNR | time
-|-|-
Gaussian-Flow[3] | 32.00 | 41.8 min
Swift4D(Ours) | 32.23 | 25.0 min



[1] SC-GS: Sparse-controlled Gaussian splatting for editable dynamic scenes. CVPR 2024.

[2] Deformable 3D Gaussians for high-fidelity monocular dynamic scene reconstruction. CVPR 2024.

[3] Gaussian-flow: 4D reconstruction with dynamic 3D Gaussian particles. CVPR 2024.

[4] 3DGStream: On-the-fly Training of 3D Gaussians for Efficient Streaming of Photo-Realistic Free-Viewpoint Videos. CVPR 2024

[5] Real-time Photorealistic Dynamic Scene Representation and Rendering with 4D Gaussian Splatting. ICLR 2024.

[6] Neural 3d video synthesis from multi-view video. CVPR 2022.







\newpage



% 5 4
% 作者提出了一种创新方法，通过引入与 Alpha 混合相结合的新颖高斯属性，将场景分解为静态和动态组件。据我所知，这是第一种利用高斯分布进行场景分解的方法。结果证明了其在所使用的数据集上的有效性，实现了高质量的渲染。


% The primary concern regarding this paper is the lack of sufficient comparisons. While the authors assert that their method is suitable for dynamic scenes, the datasets utilized predominantly feature forward-facing scenes with limited movements. Although the VRU dataset is a multi-view dataset that captures inward-looking scenes, the authors did not provide quantitative comparisons involving it. Additionally, there are other multi-view datasets [1, 2] on which Swift4D could be evaluated, particularly D-NeRF [1], which has been employed in various deformation-based dynamic neural rendering methods that could serve as points of comparison.

% The authors mention other methods, Liang et al. (2023) and He et al. (2024), that are also doing static-dynamic decomposition. However, it would be more beneficial to compare their methodologies with the proposed method through quantitative experiments rather than relying solely on qualitative descriptions.

% Furthermore, the video results from the VRU dataset exhibit noticeable abrupt scene changes, likely due to the segmentation processing of the video. The authors should address this phenomenon in the paper.

% [1] Pumarola, A., Corona, E., Pons-Moll, G., & Moreno-Noguer, F. (2021). D-nerf: Neural radiance fields for dynamic scenes. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 10318-10327). [2] Xu, Z., Peng, S., Lin, H., He, G., Sun, J., Shen, Y., ... & Zhou, X. (2024). 4k4d: Real-time 4d view synthesis at 4k resolution. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 20029-20040).

% 本文的主要担忧是缺乏足够的比较。虽然作者声称他们的方法适用于动态场景，但所使用的数据集主要具有运动有限的前向场景。尽管 VRU 数据集是捕获内向场景的多视图数据集，但作者没有提供涉及它的定量比较。此外，还有其他多视图数据集 [1, 2] 可以评估 Swift4D，特别是 D-NeRF [1]，它已被用于各种基于变形的动态神经渲染方法，可以作为比较点。

% 作者提到了其他方法，Liang 等人。 （2023）和He等人。 （2024），也在进行静态-动态分解。然而，通过定量实验将他们的方法与所提出的方法进行比较而不是仅仅依赖定性描述会更有益。

% 此外，VRU 数据集的视频结果表现出明显的场景突变，这可能是由于视频的分割处理造成的。作者应该在论文中解决这一现象。



% [1] Pumarola, A.、Corona, E.、Pons-Moll, G. 和 Moreno-Noguer, F. (2021)。 D-nerf：动态场景的神经辐射场。 IEEE/CVF 计算机视觉和模式识别会议论文集（第 10318-10327 页）。 
% [2] 徐Z.、彭S.、林H.、何G.、孙J.、沉Y.、……&周X. (2024)。 4k4d：4k 分辨率的实时 4d 视图合成。 IEEE/CVF 计算机视觉和模式识别会议论文集（第 20029-20040 页）。



% 感谢您的审稿意见，我将在这里逐一解决您的困惑，如果有任何我没有解释清楚的地方，请一定让我知道

% 1. 我们的方法聚焦多视角动态场景，所使用的数据集包括主流的 NV3D和Meetroom 数据集，这些是目前多视角方法主要测试数据集，这些数据集确实运动有限。因此为了验证我们方法的鲁棒性，我们额外在具有各种 large-scale motion 的 VRU 数据集进行测试。其定量测试结果我们在附录提供了，其结果如下：

% 2. 在 [1, 2]  数据集进行评估。由于 我们的方法和【】一样聚焦于多视角动态重建，因此无法在 D-NeRF 数据集进行测试，而[2] 使用的数据集包括 DNR-rendering，ENeRF-Outdoor , NHR. 其中 ENeRF-Outdoor 是一个单目数据集，与我们的方法不适配，DNR-rendering，NHR 主要聚焦人体细节的重建，需要将动态人体使用 mask 抠出不包含任何背景，而我们的方法是在复杂的场景下实现动态场景的重建，二者目标不同，因此不太容易进行比较。



% 3. VRU 数据集的视频结果表现出明显的场景突变。
% 因为时域结构（包括其他的动态方法，普遍存在的问题）目前无法存储太长序列的 VRU 场景信息，因此我们每隔20帧便需要重新训练一次我们的时域结构。然后将每次的渲染结果手动拼合在一起，所以就出现了每20帧一次的场景突变。因为每20帧的训练模型是不同的.



Thank you for your valuable review comments. I will address each of your concerns here. If there is anything I haven't explained clearly, please don't hesitate to let me know.

**Weaknesses:**

**W1: The primary concern regarding this paper is the lack of sufficient comparisons.**

We fully understand the reviewers' concerns. Following previous multi-view methods [3,4,5,15,16], we use the widely adopted N3DV[4] and Meetroom[5] datasets, which serve as primary benchmarks for current multi-view approaches [2,3,5,15,16]. To make our results more convincing, we also conduct experiments on the more challenging VRU dataset.
The methods we compare include recent state-of-the-art methods: SpacetimeGS[15], realtimegs[16], 3DGStream[3], 4DGS[10], and others.

In our paper, we include as many datasets and comparison methods as possible. Additionally, we have conducted experiments on the dataset you suggested, as detailed later (w3).




**W2: While the authors assert that their method is suitable for dynamic scenes, the datasets utilized predominantly feature forward-facing scenes with limited movements. The authors do not provide test results on the VRU dataset.**

In fact, most multi-view dynamic scene reconstruction methods conduct experiments on these two datasets [4,5] (which may indeed have limited movements). We follow their choice of datasets to enable direct comparison. To further demonstrate the credibility of our method, we also conduct experiments on the more challenging VRU dataset[17], which features large movements. The quantitative results are provided in the appendix (Line 798) and are as follows:

| Method                      | PSNR ↑ | SSIM ↑ | LPIPS ↓ |
|-----------------------------|--------|--------|---------|
| 4DGS [10]       | 27.87  | 0.921  | 0.191   |
| Swift4D (Ours)              | 29.03  | 0.933  | 0.187   |


**W3: There are other multi-view datasets [1, 2], particularly D-NeRF [1], on which Swift4D could be evaluated.**

These two papers include a total of five datasets: D-NeRF [1], DNR-rendering [6], NHR [7], N3DV [8], and ENeRF [9]. 


N3DV [8] is a mainstream multi-view testing dataset, and we have conducted experiments on it, as shown in our paper (line 324). As for ENeRF dataset [9], we follow the 4k4d training policy. Our results are as follows:

| Methods  | PSNR ↑   | SSIM ↑    | LPIPS ↓       |
|--|--|----|----|
| ENeRF [9]    | 25.452   | 0.809     | 0.273          |
| IBRNet [11]   | 24.966   | **0.929**     | 0.172          |
| KPlanes [13]  | 21.310   | 0.735     | 0.454          |
| 4k4d [2]    | 25.815   | 0.898     | 0.147          |
| Swift4D(Ours)     | **26.120**   | 0.911     | **0.070 (alax)**   |


As for D-NeRF [1], it is actually a monocular dataset, which is contrary to our multi-view task. DNR-rendering [6] and NHR [7] primarily focus on the reconstruction of dynamic human details, whereas we focus on the reconstruction of dynamic scenes. Humans and scenes represent two distinct tasks, so we do not conduct experiments on their datasets.
 

**W4: It is beneficial to compare the proposed method with those of Liang[13] and He[14].**

Thank you for your suggestion. We will make further qualitative comparisons in the paper.

Here, we also provide a brief introduction: Liang [13] focuses on monocular dynamic scenes, and we did not find multi-view results in their work. Additionally, since their code is not open-sourced, it is difficult for us to make a comparison. He [14] achieves a PSNR of 31.23 dB on the mainstream N3DV dataset, while ours is 32.23 dB.



**W5:  The video results from the VRU [17] dataset exhibit noticeable abrupt scene changes.**

The scene abrupt changes are caused by the way the basketball video was constructed, as it is made up of four 20-frame video clips stitched together. These abrupt changes occur at the transitions between each clip. 

Additionally, the VRU dataset is more closely related to real-life scenarios and presents significant challenges. Current dynamic methods generally suffer from flickering issues on this dataset. We have also provided the results of other methods trained on the VRU dataset in our newly added supplementary videos for comparison. Although our method also exhibits some flickering issues, it represents the scene more faithfully compared to other methods [3,10].


**Questions:**

**Q1: The scope and limitations of the proposed method are not clearly defined.**

Thank you for the reminder. Dynamic scene reconstruction can be divided into multi-view and monocular dynamic scene reconstruction, with each method presenting different challenges. The main limitation of our method is that, similar to previous work [2,3,5], it focuses on multi-view scenes and currently does not support monocular datasets for dynamic scene reconstruction. Additionally, our method focuses on scene reconstruction and does not include human reconstruction [6,7].


**Reference**

[1] D-nerf: Neural radiance fields for dynamic scenes. CVPR 2021 

[2] 4k4d: Real-time 4d view synthesis at 4k resolution. CVPR 2024.

[3] 3DGStream: On-the-fly Training of 3D Gaussians for Efficient Streaming of Photo-Realistic Free-Viewpoint Videos. CVPR 2024

[4] Neural 3d video synthesis from multi-view video. CVPR 2022.

[5] Streaming radiance fields for 3d video synthesis. NIPS 2022.

[6] DNA-Rendering. ICCV 2023.

[7] Multi-view Neural Human Rendering. CVPR 2020.

[8] Neural 3d video synthesis from multi-view video. CVPR 2022.

[9] ENeRF: Efficient Neural Radiance Fields for Interactive Free-viewpoint Video. SIGGRAPH Asia 2022

[10] 4D Gaussian Splatting for Real-Time Dynamic Scene Rendering. CVPR 2024.

[11] IBRNet: Learning Multi-View Image-Based Rendering. CVPR 2021.

[12] K-Planes: Explicit Radiance Fields in Space, Time, and Appearance. CVPR 2023.

[13] Gaufre:Gaussian deformation fields for real-time dynamic novel view synthesis. WACV 2025.

[14] S4D: Streaming 4D Real-World Reconstruction with Gaussians and 3D Control Points. Arxiv.

[15] Spacetime Gaussian Feature Splatting for Real-Time Dynamic View Synthesis. CVPR 2024.

[16] REAL-TIME PHOTOREALISTIC DYNAMIC SCENE REPRESENTATION AND RENDERING WITH 4D GAUSSIAN SPLATTING. ICLR 2024.

[17] VRU. https://anonymous.4open.science/r/vru-sequence/. 2024.

